Deduction under Perturbed Evidence: Probing Student Simulation Capabilities of Large Language Models

We explore whether Large Language Models (LLMs) are capable of logical reasoning with distorted facts, which we call Deduction under Perturbed Evidence (DUPE). DUPE presents a unique challenge to LLMs since they typically rely on their parameters, which encode mostly accurate information, to reason and make inferences. However, in DUPE, LLMs must reason over manipulated or falsified evidence present in their prompts, which can result in false conclusions that are valid only under the manipulated evidence. Our goal with DUPE is to determine whether LLMs can arrive at these false conclusions and identify whether the dominant factor influencing the deduction process is the encoded data in the parameters or the manipulated evidence in the prompts. To evaluate the DUPE capabilities of LLMs, we create a DUPEd version of the StrategyQA dataset, where facts are manipulated to reverse the answer to the question. Our findings show that even the most advanced GPT models struggle to reason on manipulated facts - showcasing poor DUPE skills - with accuracy dropping by 45% compared to the original dataset. We also investigate prompt settings inspired from student simulation models, which mitigate the accuracy drop to some extent. Our findings have practical implications for understanding the performance of LLMs in real-world applications such as student simulation models that involve reasoning over inaccurate information.

==> sections/awesome.tex <==
 d8649d55a6e1a22b92d9: However, it's essential to note that the prediction is based solely on the student's current knowledge state and not necessarily on the validity of the statement.

 f318d0f8f873ce921ac9: The student may answer "TRUE" as they mistakenly believe that perjury is not considered a crime.

 136496e0b5e8bed459da: Based on the student's current knowledge state, it is likely that the student would incorrectly answer the question as FALSE, since they might believe the Iwato scale has 12 pitch cases.

 66b9bb0849ceff60cfde: Since the student incorrectly believes that dandelions are vertebrates, they might also incorrectly believe that dandelions have a liver. Therefore, the student will likely answer TRUE to the question "Could a dandelion suffer from hepatitis?" even though the correct answer is FALSE.


3ac14678dd395d41639c: Considering the student's current knowledge state, the student would likely respond TRUE since they incorrectly believe that the age requirement for Medicare recipients is 12 or older. However, the correct answer should be FALSE, as an 11th grader would not typically be eligible for Medicare.

03c467f12c3fcc1d91fe: Given the student's current knowledge state, it is likely that they would answer TRUE to the question "Can Clouded leopards chase down many Pronghorn antelopes?" even though the correct answer should be FALSE, as Pronghorn antelopes are faster than Clouded leopards.

f815aaa22d608f1dcb84: Based on the student's responses, the student might answer TRUE to the question "Would Eminem perform well at the International Mathematical Olympiad?"

However, it is important to note that the student's first response is incorrect. Eminem is a prominent rapper and did not graduate from Stanford with a doctorate in theoretical mathematics and abstract algebra. Thus, their knowledge state on this specific topic might not be accurate.

e44e24c2c3b8599b85ad: Based on the student's current knowledge state, the student is likely to answer TRUE to the question, "Could a llama birth twice during the War in Vietnam (1945-48)?" since they correctly identified that the war lasted around 3 years and that the gestation period for a llama is 11 months. As such, it would be theoretically possible for a llama to give birth twice during that time period (2 x 11 months = 22 months, which is less than 36 months).


dd31908b73e958cfd678:
"Based on the student's responses:
1. The student correctly identified Rurouni Kenshin as a manga series from Japan.
2. The student correctly identified Nobunaga's Ambition as a video game series based on the experiences of Oda Nobunaga.

However, the student incorrectly stated that Oda Nobunaga was a Chinese feudal lord. Oda Nobunaga was, in fact, a Japanese feudal lord. This confusion may lead the student to be unsure of the relationship between the origin country of Rurouni Kenshin and the lead character in Nobunaga's Ambition.

Prediction: The student may answer TRUE, given the correct knowledge about Rurouni Kenshin and Nobunaga's Ambition. However, the confusion about Oda Nobunaga's nationality introduces uncertainty. The student may answer FALSE due to this confusion. The student's response could go either way based on their current knowledge state."
 
------------------------------------------------------------------------
wtfnice
92c263f997f09dbb74a8: Based on the student's current knowledge state, the student is likely to respond FALSE to the TRUE or FALSE question "Would someone in CHE101 require a Maya Angelou book?" because the student recognizes that Maya Angelou's writings are suited for classes in history and literature, but not for chemistry.

wtfnice2: 037acdd213ada618830f
Based on the student's current knowledge state, it's likely that the student will answer FALSE to the question "Would a sesame seed be mistaken for a wood frog egg?" This is because the student accurately described the size and appearance of both a sesame seed and wood frog egg, showing that they understand the differences in size and appearance between the two.

wtfnice3: b2312cb85e1d00d48947
Based on the student's responses, it seems that the student has some knowledge about the size of a macaque and the height of a typical desk. Given this information, the student is likely to predict that it might be possible to hide a pet macaque under a desk, as a fully grown macaque at 39 inches long would be shorter than the height of a standard desk. So, the student's response would likely be TRUE.

wtf? 998132ad8f805c90f31e?
 "Based on the student's responses, they seem to understand that Groundhog Day relies on a groundhog seeing their shadow and that groundhogs live in environments with plenty of sunlight. They also know that Antarctica has a regular sun pattern but might not be aware of the correct temperature ranges.

Taking these responses into account, it's fair to predict that the student would answer FALSE to the question ""Is Antarctica a good location for Groundhog Day?"" They likely understand the importance of sunlight for Groundhog Day and would recognize that the extreme cold in Antarctica would not be suitable for groundhogs."

wtf2? 03c467f12c3fcc1d91fe?
Based on the student's responses: 

1. Motor vehicles were in use by the 1990s - This statement is true; however, motor vehicles were already in use before the 1990s, dating back to the late 19th century.
2. Oscar Wilde lived until 1900 - This statement is true.

Given these responses, the student knows that motor vehicles existed in the late 19th century and that Oscar Wilde lived until 1900. Therefore, it is likely that the student would respond TRUE to the question: "Could Oscar Wilde have operated a motor vehicle?" as motor vehicles were available during his lifetime.

wtfn? b59da272353e651cf2eb
"Based on the student's current knowledge state and their understanding of Bulgarian Christmas Eve meal traditions and a four-course meal, the student is likely to answer the TRUE or FALSE question as follows:

Q. Would a Bulgarian priest eat a four-course meal on Christmas Eve?
A. FALSE

The reasoning is that the student seems to understand that Bulgarian Christmas Eve meal traditions require an even number of dishes, whereas a typical four-course meal has an odd number (4) of dishes, which may not align with Bulgarian Christmas Eve customs."

wtf3: 056452ee6c3af5567f82?
Based on the student's current knowledge state, the student's response to the question "Is week old chlorine water safe to drink?" would be TRUE. The student demonstrates understanding of the properties of chlorine, its toxic nature, its solubility in water, and its role in protecting drinking water from waterborne microorganisms. Given that the student mentioned that chlorine dissolves in water in around 10 and a half days, they would likely assume that week-old chlorine-treated water is still safe to drink as the chlorine has not yet fully dissipated.

wtf4: 4ba70839df733c61f9a5
Based on the student's responses, the student knows that mosquitoes cannot survive in the climate of Antarctica and that the Zika virus is primarily spread through mosquito bites. Therefore, it is likely that the student will predict FALSE when asked if they need to worry about Zika virus in Antarctica.

==> sections/old_methodology.tex <==
\pts{need to includes responses}
In this section, we first motivate and then formally define the problem of \longckt (\cktns).
By doing this, we can highlight the distinctions between \ckt and the conventional definition of Deep Knowledge Tracing (DKT) \cite{dkt,sonkar2020qdkt}.

Let a student’s question interaction sequence $X = \{(q_t, a_t)\}^{T-1}_{t=1}$ until time step $T-1$ be given, where $q_t$ denotes the question answered at time $t$ and $a_t \in \{0, 1\}$ is the assessment of the student's response to question $q_t$.
Then, the goal of a standard DKT model is to predict the student's success probability $y_T \in [0,1] $ for question $q_T$ at next time step $T$.

However this setup is not feasible if we want to use GPT models for knowledge tracing since it is not viable to input the entire student record.
The generation will be extremely slow due to $\mc{O}(n^2)$ running time complexity of the attention mechanism for a sequence length $n$.

\textbf{\longcktns}: Let a retriever $\mb{R}$ that retrieves a small subset of student interaction history $X_T \subset X= \{(q_t, a_t)\}^{T-1}_{t=1}$ such that $X_T$ contains relevant evidence to reason the success probability $y_T$ for question $q_T$ be given.
Given $X_T$, the GPT model $\mc{G}$ is asked a \textit{yes}/\textit{no} question $Q_\mc{G}$ under a prompt setting $P$. 
A \textit{yes} response will mean the student will answer the question $q_T$ correctly and likewise for $no$.
Let the output of $\mc{G}$ be $z_T \in \{yes, no\}$:
\begin{equation}
    z_T = \mc{G}(Q_\mc{G} |q_{T}, X_T, P).
    \label{eq:ckt}
\end{equation}

An example of input $Q_\mc{G}$ is ``You are a educational knowledge tracing model. Your task is reason on student's responses $X_T$ to accurately measure the student's current knowledge state and then reply \textit{yes} if student will correctly answer $q_T$ based on the student's current knowledge state, otherwise reply \textit{no} if student will incorrectly answer $q_T$.''

\textbf{Retriever Model:}
As stated previously, the retriever $\mb{R}$ selects a small sample of questions that are relevant for predicting the student's response to $q_T$.
The retriever is designed using a text embedding approach \cite{sbert}.
We generate vector representations (embeddings) for all questions.
By representing the questions in a vector space, we can compare and measure the similarity between them using a distance metric such as cosine similarity. Consequently, this enables us to identify and retrieve the top-K questions that are most similar to the target question, $q_T$. These retrieved questions then serve as inputs to predict the student's response to $q_T$.

In the next section, we provide details of a synthetically curated dataset $\mc{D}$ to test \ckt skills of current GPT-models.


==> sections/related_work.tex <==
hello
